EvSegSNN: Neuromorphic Semantic Segmentation for Event Data

Semantic segmentation is an important computer vision task, particularly for scene understanding and navigation of autonomous vehicles and UAVs. Several variations of deep neural network architectures have been designed to tackle this task. However, due to their huge computational costs and their high memory consumption, these models are not meant to be deployed on resource-constrained systems. To address this limitation, we introduce an end-to-end biologically inspired semantic segmentation approach by combining Spiking Neural Networks (SNNs, a low-power alternative to classical neural networks) with event cameras whose output data can directly feed these neural network inputs. We have designed EvSegSNN, a biologically plausible encoder-decoder U-shaped architecture relying on Parametric Leaky Integrate and Fire neurons in an objective to trade-off resource usage against performance. The experiments conducted on DDD17 demonstrate that EvSegSNN outperforms the closest state-of-the-art model in terms of MIoU while reducing the number of parameters by a factor of $1.6$ and sparing a batch normalization stage.

==> papers.tex <==
Hand-gesture recognition based on EMG and event based-camera sensors fusion: A benchmark in Neuromorphic computing: Enea Ceolini, Lyes Khacef


Spiking neural network for image segmentation: Kinjal Patel, Chris Eliasmith

Event driven visual tactile sensing and learning for robots: Tasbola Taunyazov 


\begin{table}[!htb] \label{modelsnn}
\caption{EvSegSNN architecture}
\centering
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Encoder layers}}                                                       & \multicolumn{1}{c|}{\textbf{Intermediate layers}}                                   & \multicolumn{1}{c|}{\textbf{Decoder layers}}                                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}Conv2D{[}2, 64{]}\\ Conv2D{[}64, 64{]}\\ Maxpooling(2)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Conv2D{[}256, 512{]}\\ Conv2D{[}512, 512{]}\end{tabular} & \begin{tabular}[c]{@{}l@{}}TranspConv{[}512, 256, 2{]}\\ Conv2D{[}512, 256{]} \\ Conv2D{[}256, 256{]}\end{tabular}                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Conv2D{[}64, 128{]}\\ Conv2D{[}128, 128{]}\\ Maxpooling(2)\end{tabular}  &                                                                                     & \begin{tabular}[c]{@{}l@{}}TranspConv{[}256, 128, 2{]} \\ Conv2D{[}256, 128{]} \\ Conv2D{[}128, 128{]}\end{tabular}                  \\ \hline
\begin{tabular}[c]{@{}l@{}}Conv2D{[}128, 256{]}\\ Conv2D{[}256, 256{]}\\ Maxpooling(2)\end{tabular} &                                                                                     & \begin{tabular}[c]{@{}l@{}}TranspConv{[}128, 64, 2{]} \\ Conv2D{[}128, 64{]} \\ Conv2D{[}64, 64{]} \\ Conv2D{[}64, 6{]}\end{tabular} \\ \hline
\end{tabular}
\end{table}


The SNN architecture of our reduced Unet model is detailed in Tab. \ref{modelsnn} where Conv2D[$x,y$] denotes the use of a convolution that takes as input $x$ channels and outputs $y$ channels, Maxpool($z$) denotes the use of a maxpooling with a stride equal to z, thus, dividing the frame resolution by z and TranspConv2D[$x,y,n$] denotes the use of an upsampling with a scale-factor equal to $n$, followed by a convolution that takes as input $x$ channels and returns $y$ ones. Moreover, both encoder and decoder are connected via skip connections to help deep neural architecture to avoid the vanishing gradient problem and also to make the fine-grained details learned in the encoder part used in the decoder to construct the initial image.
